Extended Equal Service and Differentiated Service Models for Peer-to-Peer File Sharing

Peer-to-Peer (P2P) systems have proved to be the most effective and popular file sharing applications in recent years. Previous studies mainly focus on the equal service and the differentiated service strategies when peers have no initial data before their download. In an upload-constrained P2P file sharing system, we model both the equal service process and the differentiated service process when peers' initial data distribution satisfies some special conditions, and also show how to minimize the time to get the file to any number of peers. The proposed models can reveal the intrinsic relations among the initial data amount, the size of peer set and the minimum last finish time. By using the models, we can also provide arbitrary degree of differentiated service to a certain number of peers. We believe that our analysis process and achieved theoretical results could provide fundamental insights into studies on bandwidth allocation and data scheduling, and can give helpful reference both for improving system performance and building effective incentive mechanism in P2P file sharing systems.

==> config.tex <==
\setvolume{x}                             %for printing use only
\setyear{2012}                             %for printing use only
\setpagerange{1}{16}                    %for printing use only
\setheadauthor{J. Zhang et al.}          %for printing use only
\setissn{1229-2370} \setpubdate{March 2012} \setno{1}

\afterpage{\beginheader}                   %for printing use only

